Smart matching

One of the most annoying aspects in the formalization of mathematics is the need of transforming notions to match a given, existing result. This kind of transformations, often based on a conspicuous background knowledge in the given scientific domain (mostly expressed in the form of equalities or isomorphisms), are usually implicit in the mathematical discourse, and it would be highly desirable to obtain a similar behavior in interactive provers. The paper describes the superposition-based implementation of this feature inside the Matita interactive theorem prover, focusing in particular on the so called smart application tactic, supporting smart matching between a goal and a given result.

==> lst-grafite.tex <==
\lstdefinelanguage{grafite} {
mathescape=true,
texcl=false,
keywords={include, set},
morekeywords={record, with, match, let, rec, corec, inductive, definition, axiom,
	qed, intro, intros, symmetry, simplify, rewrite, apply, elim, assumption,
	left, cut, cases, auto, right, coercion, split, lemma, theorem, skip,
	by, done, we, conclude, assume, need, to, prove, unfold, return, and,
	notation, interpretation, lapply, repeat, try, as, clear, in},
%emph={[1]Type, Prop, nat, real}, emphstyle={[1]\textit},
literate=	
	{->}{{$\to$}}3		
	{:>}{{$\mathrm{:>}$}}1		
	{>->}{{$\mapsto$}}2		
	{<=}{{$\leq$}}2			
	{>=}{{$\geq$}}2		
	{<>}{{$\neq$}}1
	{\\/}{{$\vee$}}1 		
	{<->}{{$\leftrightarrow$}}2
	{FORALL\ }{{$\forall\,$}}1		
	{EXISTS\ }{{$\exists\,$}}1
	{ALPHA}{{$\alpha$}}1
	{LAMBDA}{{$\lambda\,$}}1
	{LANGLE}{{$\langle$}}1
	{RANGLE}{{$\rangle$}}1
	{EQUIV}{{$\equiv$}}1
	{SIGMA}{{$\Sigma$}}1
	{PSI}{{$\Psi$}}1
	{DOTS}{{$\ldots$}}1
	{NOT}{{$\neg$}}1
	{\\in}{{$\in$}}1
	{/\\}{$\land$}1
	{=>}{{$\,\Rightarrow\,$}}1
	{≝}{{:=}}1
	{δ}{{$\delta$}}1
	{λ}{{$\lambda\,$}}1
	{≰}{{$\nleq\,$}}1
	{∨}{{$\lor\,$}}1
	{≈}{{$\approx\,$}}1
	{∀}{{$\forall\,$}}1
	{∃}{{$\exists\,$}}1
	{⇝}{{$\leadsto\,$}}1
	{→}{{$\rightarrow\,$}}1
	{∧}{{$\land\,$}}1
	{≤}{{$\leq\,$}}1
	{¬}{{$\lnot\,$}}1
	{≪}{{$\ll\,$}}1
	{≫}{{$\gg\,$}}1
	{⇒}{{$\,\Rightarrow$}}1
	{⊢}{{$\vdash$}}1
	{...}{{$\ldots$}}1
	,
comment=[s]{(*}{*)},
showstringspaces=true,
extendedchars=true,
sensitive=false,
captionpos=b,
mathescape=true,
%backgroundcolor=\color{gray},
frame=tblr,
frameround=tttt,
columns=flexible,
basicstyle=\small,
}


